Elliptic Curve Based Zero Knowledge Proofs and Their Applicability on Resource Constrained Devices

Elliptic Curve Cryptography (ECC) is an attractive alternative to conventional public key cryptography, such as RSA. ECC is an ideal candidate for implementation on constrained devices where the major computational resources i.e. speed, memory are limited and low-power wireless communication protocols are employed. That is because it attains the same security levels with traditional cryptosystems using smaller parameter sizes. Moreover, in several application areas such as person identification and eVoting, it is frequently required of entities to prove knowledge of some fact without revealing this knowledge. Such proofs of knowledge are called Zero Knowledge Interactive Proofs (ZKIP) and involve interactions between two communicating parties, the Prover and the Verifier. In a ZKIP, the Prover demonstrates the possesion of some information (e.g. authentication information) to the Verifier without disclosing it. In this paper, we focus on the application of ZKIP protocols on resource constrained devices. We study well-established ZKIP protocols based on the discrete logarithm problem and we transform them under the ECC setting. Then, we implement the proposed protocols on Wiselib, a generic and open source algorithmic library. Finally, we present a thorough evaluation of the protocols on two popular hardware platforms equipped with low end microcontrollers (Jennic JN5139, TI MSP430) and 802.15.4 RF transceivers, in terms of code size, execution time, message size and energy requirements. To the best of our knowledge, this is the first attempt of implementing and evaluating ZKIP protocols with emphasis on low-end devices. This work's results can be used from developers who wish to achieve certain levels of security and privacy in their applications.

==> zkpdl.tex <==
\section{Zero Knowledge Proofs Based on DLP}

A wide variety of zero-knowledge protocols based on the Discrete Logarithm Problem 
(DLP) has been proposed so far, e.g. in \cite{Smith05cryptographymeets}.  
Consider a finite cyclic group $F$ of order $n$ with a generator $g$, for example 
the multiplicative group $Z_{n}^{*}$ of order $n-1$ where the group operation is multiplication modulo $n$.
The Discrete Logarithm Problem (DLP) can be defined as follows:
Given a prime $n$, a generator $g$ of $Z_{n}^{*}$ and an element $b \in Z_{n}^{*}$, find the integer 
$x$, $ 0 \leq x \leq n-2$ such that $g^x = b (mod \, n)$ \cite{548089}. 
Next, we describe well-established zero-knowledge protocols of this category. 

\subsection{Zero Knowledge Proof of Discrete Logarithm with Coin Flip}

One of the first zero knowledge protocols of discrete logarithm that was originally 
presented in \cite{springerlink:10.1007/3-540-39118-5_13}.
The Prover wants to prove in zero-knowledge that he knows the discrete
logarithm of a given number modulo $n$ (the order of the group $F$). 
Given a generator $g$ for $F$ and $b \in F$, the Prover aims at proving that he knows $x$
such that $g^x = b (mod \, n)$ without revealing $x$. Initially, both Prover and Verifier 
know generator $g$ as well as $b$ but the Prover also knows $x$, the discrete logarithm of $b$.

\textbf{Protocol Steps :}
\begin{itemize}
\item Prover generates random $r \in {1, ... , n-1}$ and computes $h = g^r (mod \, n)$
\item Prover sends $h$ to Verifier
\item Verifier flips a coin and informs the Prover about the outcome
\item In case of HEADS Prover sends $r$ to Verifier who checks that $g^r = h$
\item In case of TAILS Prover sends $m = x + r (mod \, n - 1)$ to Verifier who checks that $g^m (mod \, n)= g^{(x+r)}(mod \, n) = g^x \cdot g^r(mod \, n) = b \cdot h$
\end{itemize}

The above steps are repeated until Verifier is convinced that Prover knows 
$x$ with probability $1 - 2^{-k}$ for $k$ iterations.

\textbf{Why it works :} The above protocol works as expected because
in each iteration the steps to be executed depend on the outcome of
the coin that the Verifier flips and the Prover cannot affect this.
Thus, a dishonest Prover in each iteration can prepare for only one
of the coin outcomes. For example, if he prepares for TAILS, he can
cheat by generating random $m$, computing $h = (g^m) / b (mod \, n)$
and sending $h$ to Verifier. This attack works if the coin is TAILS
but does not work for HEADS as the Prover would have to find $r$ out
of $h$, which is computationally hard according to the discrete
logarithm problem. Similarly, if a dishonest Prover prepares for
HEADS generating random $r$ and computing $h$, he can successfully
answer in case of HEADS but not in case of TAILS if he does not know
$x$ the discrete logarithm of $b$.

Conclusively, a Prover has $1/2$ probability of cheating in each
iteration. By repeating the protocol steps for $k$ times the
cheating probability is $2^{-k}$ which becomes very small as the $k$
grows. Thus, by repeating the protocol steps many times the Verifier
can be assured that the Prover is not cheating.

\subsection{Schnorr's Protocol}

An improvement of the previous protocol was originally presented in \cite{springerlink:10.1007/BF00196725}. 
The Prover and the Verifier know a generator $g$ as well as $b$ an element of the group $F$. 
Prover claims that he knows $x$ the discrete logarithm of $b$ such that $g^x= b (mod \, n)$.
He wants to prove this to Verifier without revealing $x$.

\textbf{Protocol Steps :}
\begin{itemize}
\item Prover generates random $r \in {1, ..., n-1} $ and computes $h= g^r (mod \, n)$
\item Prover sends $h$ to Verifier
\item Verifier computes random $c \in {1, ..., n-1} $ and sends $c$ to Prover
\item Prover computes $m= r + c \cdot x (mod \, n - 1)$ and sends $m$ to Verifier
\item Verifier checks that  $t = g^m / b^c (mod \, n) = g^{(r+c \cdot x)} / b^c (mod \, n) \\ = (g^r \cdot g^{cx}) / b^c (mod \, n)= g^r (mod \, n)= h$
\end{itemize}

\textbf{Why it works :} In this protocol, in correspondence with the
previous one, Verifier's coin flips are simulated by replying with
a random value $c$. That is the reason for which this protocols requires only
one round of execution. A dishonest Prover has a tiny chance of
cheating as he would have to fix the value of $t= g^m / b^c$ before
receiving Verifier's random value $c$. Under the assumption that the
random number generator used by the Verifier is secure, a Prover who does not
know $x$, the discrete logarithm of $b$, cannot cheat.

\subsection{Transforming Schnorr's Protocol to Digital Signature}

In \cite{Fiat:1987:PYP:36664.36676}, the authors propose that with the use of a
hash function and an agreement on an initial message $m$ one can remove the 
interactivity from such protocols. The Verifier's random choices can be replaced 
with bits produced by a secure hash function. Thus, the next protocol is proposed.

Prover and Verifier know generator $g$ and element $b$ in the group $F$ of order $n$. 
Prover claims that he knows $x$ the discrete logarithm of $b$ such that $g^x = b (mod \, n)$
and wants to prove this to Verifier without revealing $x$. They both agree on a hash 
function HASH (e.g. SHA-1). Moreover, in an offline step Prover and Verifier agree on value $m$ that represents a message.

\textbf{Protocol Steps :}
\begin{itemize}
\item Prover generates random $r \in {1, ... , n-1}$ and computes $h = g^r (mod \, n)$
\item Prover computes $c= HASH(m^x (mod \, n), m^r (mod \, n),\\ g^r (mod \, n))$
\item Prover computes $s = r + c \cdot x (mod \, n)$ and sends to Verifier the following message : \\ ``$s || m^x (mod \, n) || m^r (mod \, n) || g^r (mod \, n)$''
\item Verifier computes $c= HASH(m^x (mod \, n), m^r (mod \, n),\\ g^r (mod \, n))$
\item Verifier checks that $g^s (mod \, n)= g ^{(r+c \cdot x)}(mod \, n)= (g^r) \cdot (g^x)^{c} (mod \, n)= h \cdot b^c (mod \, n)$
\item Verifier checks that $m^s (mod \, n)= m ^{(r+c \cdot x)}(mod \, n)= (m^r) \cdot (m^x)^{c} (mod \, n)$
\end{itemize}

\textbf{Why it works :} In this protocol the Prover simulates both
the Prover and the Verifier and he publishes the transcript of this
whole dialogue. The Prover generates a random number as in previous
protocols but the Verifier's random choices are simulated by hashing
the input and a value calculated from the Prover's choice of $r$.
Thus, the Verifier's choice depends on Prover's choice and it is
made hard to fake the outcome. The value $c$ is really a challenge
for the Prover as it is computed from the hash function and it is
out of his control. If the Prover does not know $x$, in order to
cheat he would try to find $s$ satisfying $g^s (mod \, n)= (g^x)^c
\cdot g^r (mod \, n)$ which is an instance of the discrete logarithm
problem. He could not cheat by enumerating random $r$ values, as it
would be too hard to find a matching value $c$.

\subsection{Zero Knowledge Test of Discrete Logarithm Equality}

Suppose that Prover knows two publicly known quantities that have
the same discrete logarithms $x$ to publicly known respective bases
$g$ and $h$ of the group $F$. 
Prover claims that he knows $x$ the discrete logarithm of $b$
and $c$ such that $g^x = b (mod \, n)$ and $h^x = c (mod \, n)$. He
wishes to convince Verifier of this without revealing $x$. The procedure
as proposed in \cite{DBLP:conf/crypto/BoyarCDP90}, is as follows:

\textbf{Protocol Steps :}
\begin{itemize}
\item Prover generates random $r \in {1, ..., n-1}$ and computes $k=g^r (mod \, n)$ and $l=h^r(mod \, n)$
\item Prover sends $k,l$ to Verifier
\item Verifier generates random $z \in {1, ..., n-1}$ and sends $z$ to Prover
\item Prover computes $m= r + z \cdot x (mod \, n -1)$ and sends $m$ to Verifier
\item Verifier checks that $g^m (mod \, n) = g^{(r+z \cdot x)} (mod \, n) = g^r \cdot (g^x)^{z} (mod \, n) = k \cdot b^z (mod \, n)$
\item Verifier checks that $h^m (mod \, n) = h^{(r+z \cdot x)} (mod \, n) = h^r \cdot (h^x)^{z} (mod \, n) = l \cdot c^z (mod \, n)$
\end{itemize}

\textbf{Why it works :} This protocol is quite similar with the
classic zero-knowledge proof of discrete logarithm but involves two
publicly known quantities that have the same discrete logarithm. This way
the actions held by the Prover and Verifier are corresponding with
those of Schnorr's protocols, for each quantity. Additionally this
protocol can be made non-interactive using the trick proposed by Fiat and Shamir: 
the Prover simulates the Verifier by computing $z$ with a secure hash function
as HASH(b,g,c,h,k,l).

\subsection{Zero Knowledge Proof of Single Bit}

Let the large prime $n$ and generators $g,h$ of the group $F$ be public. Prover
chooses random $r \in {1, ..., n-1}$ and publicizes $b = g^r \cdot h^{\pm 1} (mod \,
n)$. He wishes to convince Verifier that he really does know $r$ and
that the exponent of $h$ really is $\pm 1$ without revealing $r$ nor
the sign bit \cite{Smith05cryptographymeets}.

\textbf{Protocol Steps:}
\begin{itemize}
\item Prover chooses random $s,d,w \in {1, ..., n-1}$
\item Prover computes $a = g^s \cdot (b \cdot h^{\pm 1})^{-d} (mod \, n)$ and $c= g^w (mod \, n)$
\item If $-1$ Prover swaps $a \leftrightarrow c$
\item Prover sends $a,c$ to Verifier
\item Verifier chooses random $z$ and sends it to Prover
\item Prover computes $e = z - d$ and $t= w + r \cdot e$ both $mod \, n - 1$
\item If $-1$ Prover swaps $ d \leftrightarrow e$ and $s \leftrightarrow t$
\item Prover sends to Verifier $d,e,s,t$
\item Verifier checks that $z = d + e$, $g^s (mod \, n) = a \cdot (bh)^{d} (mod \, n)$ and that $g^t (mod \, n) = c \cdot (bh^{-1})^{e} (mod \, n)$
\end{itemize}

\textbf{Why it works:} It is straightforward to confirm that if $b$
is really given by one of the two formulas the Prover claimed then
Verifier's verification will succeed. It is also easy to see that
the Prover does not give away any information that would allow the
Verifier to deduce $r$ nor the sign bit. That is because he
\textit{hides} $r$ inside $t$ and with the appropriate swaps in case
of $-1$ he randomizes the sign bit.
